Studying the Inductive Biases of RNNs with Synthetic Variations of Natural Languages

How do typological properties such as word order and morphological case marking affect the ability of neural sequence models to acquire the syntax of a language? Cross-linguistic comparisons of RNNs' syntactic performance (e.g., on subject-verb agreement prediction) are complicated by the fact that any two languages differ in multiple typological properties, as well as by differences in training corpus. We propose a paradigm that addresses these issues: we create synthetic versions of English, which differ from English in one or more typological parameters, and generate corpora for those languages based on a parsed English corpus. We report a series of experiments in which RNNs were trained to predict agreement features for verbs in each of those synthetic languages. Among other findings, (1) performance was higher in subject-verb-object order (as in English) than in subject-object-verb order (as in Japanese), suggesting that RNNs have a recency bias; (2) predicting agreement with both subject and object (polypersonal agreement) improves over predicting each separately, suggesting that underlying syntactic knowledge transfers across the two tasks; and (3) overt morphological case makes agreement prediction significantly easier, regardless of word order.

==> cases_example.tex <==
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Order} & \textbf{Unambiguous cases}                     & \textbf{Ambiguous cases}                       & \textbf{Argument marking (single pair)}        \\ \hline
\textbf{VOS}   & droppedkarker 190 pointker the stock marketkar & droppedkarkar 190 pointkar the stock marketkar & droppedkerkin 190 pointker the stock marketkin \\ \hline
\textbf{OSV}   & 190 pointker the stock marketkar droppedkarker & 190 pointkar the stock marketkar droppedkarkar & 190 pointker the stock marketkin droppedkerkin \\ \hline
\textbf{SOV}   & the stock marketkar 190 pointker droppedkarker & the stock marketkar 190 pointkar droppedkarkar & the stock marketkin 190 pointker droppedkerkin \\ \hline
\end{tabular}

\caption{\label{tbl:cases-example} Different combination of case systems and word orders. Original sentence is "The stock market dropped 190 points". \sr{This example is not so good for the last column (argument marking), since it has only one verb. Maybe better change to a little longer sentence?)}}


==> polypersonal_results_lemmatized.tex <==

\begin{tabular}{c|c|c}
\hline
\textbf{Agreement} & \multicolumn{1}{c|}{\textbf{Subject accuracy}} & \textbf{Object accuracy / recall} \\ \hline
\textbf{subject}   & 94.4\pm0.23                                      & -                                 \\ \hline
\textbf{object}    & -                                              & 88.3\pm$0.48 / 81.0\pm$3.6              \\ \hline
\textbf{All}       & 95.6$\pm$0.34                                      & 89.2\pm$0.61/82.9\pm$2.8               
\end{tabular}

\caption{\label{tbl:polypersonal-lemmatized} Accuracy and recall results for polypersonal agreement prediction with lemmatized verbs. "All" refers to predicting all three arguments.}



==> polypersonal_results_verbs_intact.tex <==
\begin{tabular}{c|c|c}
\hline
\textbf{Agreement} & \multicolumn{1}{c|}{\textbf{Subject accuracy}} & \textbf{Object accuracy / recall} \\ \hline
\textbf{subject}   & 94.6$$\pm$$0.25                                      & -                                 \\ \hline
\textbf{object}    & -                                              & 88.6$$\pm$$0.52 / 83.3$$\pm$$1.86             \\ \hline
\textbf{All}       & 95.6$$\pm$$0.16                                      & 89.0$$\pm$$0.19 / 81.6$$\pm$$1.06            
\end{tabular}
\caption{\label{tbl:polypersonal-intact} Accuracy and recall results for polypersonal agreement prediction with original verbs. ``All" refers to predicting all three arguments.}

